Autonomous robotic re-alignment for face-to-face underwater human-robot interaction

The use of autonomous underwater vehicles (AUVs) to accomplish traditionally challenging and dangerous tasks has proliferated thanks to advances in sensing, navigation, manipulation, and on-board computing technologies. Utilizing AUVs in underwater human-robot interaction (UHRI) has witnessed comparatively smaller levels of growth due to limitations in bi-directional communication and significant technical hurdles to bridge the gap between analogies with terrestrial interaction strategies and those that are possible in the underwater domain. A necessary component to support UHRI is establishing a system for safe robotic-diver approach to establish face-to-face communication that considers non-standard human body pose. In this work, we introduce a stereo vision system for enhancing UHRI that utilizes three-dimensional reconstruction from stereo image pairs and machine learning for localizing human joint estimates. We then establish a convention for a coordinate system that encodes the direction the human is facing with respect to the camera coordinate frame. This allows automatic setpoint computation that preserves human body scale and can be used as input to an image-based visual servo control scheme. We show that our setpoint computations tend to agree both quantitatively and qualitatively with experimental setpoint baselines. The methodology introduced shows promise for enhancing UHRI by improving robotic perception of human orientation underwater.

==> TextFiles/acknowledgments.tex <==
\section*{Acknowledgment}
This work is indebted to the entire Interactive Robotics \& Vision Laboratory (IRVLab), specifically, Jungseok Hong, Chelsey Edge, and Corey Knutson for assisting in data collection that made F2F possible. Also, a special thanks must be given to Junaed Sattar for his conscientious guidance and support throughout the development of the F2F concept.

==> TextFiles/human_analysis.tex <==
\section{Human analysis of alignment}
While the preceding analysis is intuitive, it is based on the authors' own
understanding of a human's facing direction. To that end, since the alignment
vector is a convention, we gauge the extent to which the alignment
vector agrees with other people's understanding of a person's ``facing direction." Understanding
this elucidates two things: how good are people at quantifying a person's facing direction, and what are the error bounds within which any alignment vector could be a suitable choice for a person's facing direction.

We do this by conducting a limited human study that measures agreement
between the alignment vector produced from the analysis in Section~\ref{sec:alignment}
and perturbations of the alignment vector within error bounds. Our results show that
humans struggle to quantify a person's facing direction, which effectively lifts the constraints for the control scheme that must anti-align the coordinate systems between the robot's camera frame and the diver's body frame.

The study was conducted using 13 participants, none of whom were given instruction on the overall goal of the project. They were told that they would be shown a series of images and corresponding three dimensional reconstructions along with a series of four arrows, labeled A through D. The participants were asked to use their intuition and general concepts of a person's facing direction to select from the arrow choices the arrow that they felt best represented the direction a human was facing. The arrow alternatives were computed by first computing the spherical coordinate representation of the alignment vector as $(\rho=1, \theta_{\text{GT}}, \phi_{\text{GT}})$. Then, the angles were perturbed by selecting from a uniform random distribution over the ranges
$\theta_{\text{NEW}} \in [\theta_{\text{GT}}-\theta_{\text{lBnd}}, \theta_{\text{GT}}+\theta_{\text{uBnd}}]$ and $\phi_{\text{NEW}} \in [\phi_{\text{GT}}-\phi_{\text{lBnd}}, \phi_{\text{GT}}+\phi_{\text{uBnd}}]$. Three angle bounds were sampled and chosen for both the lower bound and the upper bound (represented as a subscript ``lBnd" and ``uBnd," respectively). 

The participants were shown a total of 54 plots in three different phases. Each phase contained 18 images and corresponding three dimensional reconstruction. Each of the six canonical poses was sampled three times, which included prone facing the bottom, prone facing the surface, upright facing away from the camera, upright facing the camera, inverted facing the camera, and inverted facing away from the camera. The participants were shown both the raw grayscale camera image obtained from the left camera from the stereo pair and the corresponding three-dimensional reconstruction of the torso keypoints with the alignment vector and the three alternatives shown. The arrows were different colors but labeled from the set $\{\text{A}, \text{B}, \text{C}, \text{D}\}$ to help differentiate between arrows when the orientation would not permit clear separations. An example survey question is shown in Fig.~\ref{fig:example_survey}. 

\begin{figure}[t]
\includegraphics[width=1.0\columnwidth]{figure121268_AngleIs25_CorrectIsB_EDITED_Cropped}
\caption{(Color online) Example survey question in which the alignment vector is shown as ``B (green)". Participants were asked to select from the options the arrow that best represented the diver's facing direction.}
\label{fig:example_survey}
\end{figure}

The elevation angle $\theta$ and the azimuthal angle $\phi$ were $25^{\circ}$ in the first case, $15^{\circ}$ in the second case, and $5^{\circ}$ in the third case. In the table below we show the average number of correct judgements with the standard deviation, as well as Fleiss' $\kappa$ measurement to gauge inter-rater reliability. 

\begin{table}
\begin{center}
\caption{Summary of results for human analysis of alignment.}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 $\boldsymbol{\pm \theta,\phi}$ & \textbf{Mean (}$\boldsymbol\mu$\textbf{)} & \textbf{Standard deviation (}$\boldsymbol\sigma$\textbf{)} & $\boldsymbol\kappa$\\
 \hline
 $25^{\circ}$ & 0.327 & 0.421 & 0.080 \\ 
 $15^{\circ}$ & 0.167 & 0.324 & 0.013 \\ 
$5^{\circ}$ & 0.241 & 0.413 & 0.016 \\ 
 % $25^{\circ}$ & \hl{mean} & \hl{std} & \hl{alpha} \\
 % $15^{\circ}$ & \hl{mean} & \hl{std} & \hl{alpha} \\
 % $5^{\circ}$ & \hl{mean} & \hl{std} & \hl{alpha} \\
 \hline
\end{tabular}
\end{center}
\end{table}

 % $TODO Uncomment for journal article
% In the table below, we show the same statistics but relative to the individual poses. Clearly, we observe that in the case of \hl{INSERT DISCUSSION ABOUT WHICH POSES CAUSE THE MOST CONFUSION}.
% \begin{table*}[ht]
% \caption{Summary of results for human analysis of alignment per pose}
% \begin{center}
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{\textbf{Pose}}&\multicolumn{3}{|c|}{$\boldsymbol{\theta, \phi \pm25^{\circ}}$}&\multicolumn{3}{|c|}{$\boldsymbol{\theta, \phi \pm15^{\circ}}$}&\multicolumn{3}{|c|}{$\boldsymbol{\theta, \phi \pm5^{\circ}}$} \\\cline{2-10}
%     & $\mu$ & $\sigma$ & $\kappa$ & $\mu$ & $\sigma$ & $\kappa$ & $\mu$ & $\sigma$ & $\kappa$\\
%     \cline{1-10}
%     % Upright (Facing the camera) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\
%     % Upright (Facing away from the camera) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\
%     % Inverted (Facing the camera) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\
%     % Inverted (Facing away the camera) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\    
%     % Prone (Facing the bottom) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\
%     % Prone (Facing the surface) & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} & \hl{mean} & \hl{std} & \hl{alpha} \\       
%     Prone (surface) & 0.421 & 0.507 & 0.065 & 0.205 & 0.320 & 0.027 & 0.222 & 0.411 & 0.048 \\ 
% Prone (bottom) & 0.228 & 0.311 & 0.116 & 0.231 & 0.391 & -0.015 & 0.278 & 0.458 & -0.002 \\ 
% Upright (away) & 0.333 & 0.448 & 0.087 & 0.103 & 0.239 & 0.004 & 0.167 & 0.357 & -0.026 \\ 
% Upright (facing) & 0.421 & 0.501 & 0.063 & 0.205 & 0.410 & 0.147 & 0.194 & 0.364 & 0.027 \\ 
% Inverted (facing) & 0.158 & 0.284 & 0.127 & 0.077 & 0.277 & -0.019 & 0.222 & 0.411 & -0.029 \\ 
% Inverted (away) & 0.404 & 0.475 & 0.022 & 0.179 & 0.306 & -0.067 & 0.361 & 0.475 & 0.076 \\ 
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:multicol}
% \end{table*}


% Statistics for the Prone (surface) orientation across 9 participants are: mean 0.222 std 0.425
% Statistics for the Prone (down) orientation across 9 participants are: mean 0.333 std 0.489
% Statistics for the Upright (away) orientation across 9 participants are: mean 0.111 std 0.258
% Statistics for the Upright (facing) orientation across 9 participants are: mean 0.185 std 0.287
% Statistics for the Inverted (facing) orientation across 9 participants are: mean 0.259 std 0.444
% Statistics for the Inverted (away) orientation across 9 participants are: mean 0.370 std 0.498

% These results can be interpreted in a few ways. The poses which cause the most confusion or disagreement among the raters indicate that the human has trouble identifying which alignment vector is proper for quantifying the facing direction, but these poses could also indicate that the error bars on alignment are much more forgiving, since any control scheme must decide when to stop. From our study, it is clear that the control scheme must align to at least within \hl{INSERT THE ANGLE EXTRACTED FROM THE ANALYSIS}. Alternatively, the alignment vector convention described in this work does tend to agree with what human's believe the facing direction is. While this is by no means prescriptive, it does indicate that we have at least developed a method that agrees with what human's believe is the facing direction.
